Towards Fixing Clever-Hans Predictors with Counterfactual Knowledge Distillation

This paper introduces a novel technique called counterfactual knowledge distillation (CFKD) to detect and remove reliance on confounders in deep learning models with the help of human expert feedback. Confounders are spurious features that models tend to rely on, which can result in unexpected errors in regulated or safety-critical domains. The paper highlights the benefit of CFKD in such domains and shows some advantages of counterfactual explanations over other types of explanations. We propose an experiment scheme to quantitatively evaluate the success of CFKD and different teachers that can give feedback to the model. We also introduce a new metric that is better correlated with true test performance than validation accuracy. The paper demonstrates the effectiveness of CFKD on synthetically augmented datasets and on real-world histopathological datasets.

==> sections/future_work.tex <==
\section{Future Work}

%The proposed approach can be extended to a broader range of datasets, such as additional pathology datasets, ophthalmology datasets, or other safety-critical domains like autonomous driving. These datasets should provide high-quality images with similar characteristics to those used in the present study. This extension would facilitate the assessment of the generalizability and robustness of the approach across various domains.

The approach can also be adapted for use with other modalities, such as large language models, using the optimus framework. This adaptation may allow the approach to combat hallucination in language models, which is a significant challenge for the field. This extension would enable the application of the proposed approach to a wider range of machine learning applications beyond image classification.

Alternative generative models, such as diffusion models, could be explored for building counterfactuals. Such models may be more suitable for complex datasets with stronger modes, and may offer a more efficient approach to building counterfactuals. This extension would compensate for any weaknesses in the current generative model and could lead to more accurate and efficient identification of counterfactuals.

==> sections/limitations.tex <==
\section{Limitations}

The identification of counterfactuals can be challenging due to the limitations of gradient-based optimization. Specifically, gradient search is only capable of finding the global optimum for convex functions, which may not accurately reflect the non-convex nature of transitions between different classes.
%This issue is particularly pronounced for discrete objects in image data, which are characterized by hard class boundaries.
%Additionally, the use of normalizing flows exacerbates this problem by further complicating the identification of appropriate counterfactuals.

%Certain counterfactuals may not be easily interpretable by humans and do not necessarily adhere to traditional adversarial attack principles. Specifically, some counterfactuals may not involve any perceivable changes in the image that humans would detect. Rather, minor adjustments to insignificant features (e.g., background intensity) can be enough to trigger a change in classification. As a result, counterfactual generation can sometimes obscure the underlying process and result in unpredictable, nonlinear decision boundaries.

Not all counterfactuals accurately reflect the most salient features of the models being analyzed. Even though confounders are often considered the most important features, counterfactuals may arbitrarily remove other features that do not significantly contribute to the classification process. While these counterfactuals may still be effective in flipping the classifier's decision, they may not accurately expose to the user the different level of feature relevance.
%This issue may arise due to limitations in the generative model used to identify counterfactuals.

%Improvements in test accuracy resulting from counterfactual generation may be unstable, likely due to the aforementioned issues.

%The accuracy of feedback received during the counterfactual generation process is not always reliable, potentially due to the complex and nonlinear nature of the generated counterfactuals.

%Finally, the process of generating counterfactuals can be computationally intensive and time-consuming.
